Influence Maximization with Bandits

We consider the problem of \emph{influence maximization}, the problem of maximizing the number of people that become aware of a product by finding the `best' set of `seed' users to expose the product to. Most prior work on this topic assumes that we know the probability of each user influencing each other user, or we have data that lets us estimate these influences. However, this information is typically not initially available or is difficult to obtain. To avoid this assumption, we adopt a combinatorial multi-armed bandit paradigm that estimates the influence probabilities as we sequentially try different seed sets. We establish bounds on the performance of this procedure under the existing edge-level feedback as well as a novel and more realistic node-level feedback. Beyond our theoretical results, we describe a practical implementation and experimentally demonstrate its efficiency and effectiveness on four real datasets.

==> Experiments.tex <==
\section{Experiments}
\label{sec:Experiments}

\subsection{Influence Maximization Oracle}
For our CMAB framework, we assume the existence of an ($\alpha-\beta$) influence maximization oracle. We instantiate the oracle using the Two phase Influence Maximization(TIM) algorithm proposed recently in~\cite{Tang2014Influence}. TIM acts as a ($1 - \frac{1}{e}, 1 - \frac{1}{|E|}$) and has a near optimal run-time. We briefly describe this algorithm as follows. Given a budget of $k$ seeds, a network with $m$ edges and $n$ nodes and an appropriate diffusion model such as IC, TIM obtains a $(1 - 1/e - \epsilon)$ fraction of the optimal spread in the non-adaptive case, incurring a near-optimal runtime complexity of $\mathcal{O}(k+l)(n + m) log n / \epsilon^{2}$. TIM operates by generating a large number of random Reverse Reachable (RR) sets. An RR set is defined for a particular node $v$ and a possible world $W$ of the network. It consists of the set of nodes that can reach the node $v$ in the possible world $W$. Given enough number (see \cite{Tang2014Influence} for an explicit bound) of RR sets, the nodes which cover a large number of RR sets are chosen as the seed nodes: the node $u$ which appears in the maximum number of RR sets is chosen as the first seed. Once a node $u$ is selected as a seed, we remove all the RR sets containing $u$ and the next seed is the node which covers the maximum of the remaining RR sets and so on until a seed set $S$ with $k$ nodes is chosen. Tang et al.~\cite{Tang2014Influence} show that this simple strategy is enough to guarantee a $(1 - 1/e - \epsilon)$-approximation factor in near optimal time. 

\subsection{Prior on Influence Probabilities}
For typical social networks, we may have an idea on the range of influence probabilities. E.g., we may know that the influence probabilities lie in the range of $[0.0005, 0.2]$ for a given network. If available, we can use this domain specific information to better initialize the influence probability estimates. For the maximum likelihood approach, these initial estimates can prove to be important for faster convergence of the gradient descent method. For the frequentist (both edge level and node level approaches), where the updates are binary i.e. the $X_{i,t}$ follow a Bernoulli distribution the initialization can be treated as a Beta prior characterized  by the parameters $\alpha$ and $\beta$ the mean of which can be given by: $\frac{\alpha}{\alpha + \beta}$.  The Bernoulli and Beta distributions are conjugate priors and the posterior follows a Beta distribution. The mean of the posterior which results in a modified update rule given by: \textbf{$\hat{\mu_{i}}$} = $\frac{\sum_{s = 1}^{t}X_{i,s} + \alpha}{T_{i,t} + \alpha + \beta}$. Hence the Beta prior parameters act like pseudo counts in the update formula. This technique known as Laplace smoothing is commonly used in NLP. We show the benefit of putting a prior on the influence probabilities in section~\ref{sec:Experiments}. 

\subsection{Datasets}
We use 3 datasets - NetHept, Epinions and Flickr for our experiments. Essential properties of these datasets are summarized in table~\ref{tab:datasets}. The ``true'' probabilities for each of these datasets are set according to the weighted cascade model~\cite{kempe2003maximizing} i.e for edges into the node $v$, the influence probability is $\frac{1}{N_{in}(v)}$ where $N_{in}(v)$ is the number of in-neighbours of $v$. This constitutes our graph $G = (V,E,P)$. The learnt probabilities are initialized to 0 or set according to some available prior information. 

\begin{table}[!ht]
\centering
\begin{tabular}{ | l | c | r | r | r | }
\hline
Dataset & |V| & |E| & Av.Degree & Max.Degree \\
\hline
NetHEPT & 15K & 31K & 4.12 & 64 \\
\hline
Epinions & 76K & 509K & 13.4 & 3079 \\
\hline
Flickr & 105K & 2.3M & 43.742  &  5425 \\
\hline
\end{tabular} 
\label{tab:datasets}
\caption{Dataset characteristics}
\end{table}

\subsection{Experimental Setup}
We simulate the diffusion in the network by sampling a deterministic world from the true probabilistic graph $G$ i.e. for purpose of our experiments, we assume that the diffusion trace in the real world happened according to this deterministic graph. For this, we sample each edge in the graph according to its ``true'' probability. We vary the size of the seed set or budget $k$ from $10$ to $100$. For our influence maximization oracle, we use the TIM algorithm described earlier with $\epsilon = 0.5$. Runtime constraints dictate us to use a relatively higher value of $\epsilon$. We have verified that a smaller, more accurate value of $\epsilon$ gives us qualitatively similar results. We run the bandit algorithm for a total of $1000$ rounds and exhaust the budget $k$ in each round. For each round, we find the ``true'' spread obtained i.e. the spread obtained if the diffusion had occurred according to the deterministic graph generated. We find this value with the learnt probabilities as well as the ``true'' probabilities. Thus we are able to calculate the regret in each round of the process. We also plot the relative $L_{2}$ difference between the true and the learnt probabilities. In addition to this, we also plot the fraction of edges $f$ within a relative error of $p = 10 \%$ and plot $f$ as $p$ is varied. All our results are those obtained by averaging across $3$ runs. 

\begin{table}[!ht]
\centering
\begin{tabular}{ | l | c | r | r | r | r |}
\hline

Dataset & Explore & Explore &  \multicolumn{3}{|c|}{Update} \\
\hline
 &  & & EL & NL-F  & NL-ML \\
\hline
NetHEPT & 2.682 s & 0.0002 s & 0.0260 s & 0.0274534 s & 1.1476563 s \\
\hline
Epinions & 245.225  &  0.0014  &    &   0.224 & 15.156 \\
\hline
Flickr &  	    &         &        &           &           \\
\hline
\end{tabular} 
\label{tab:runtimes}
\caption{Subroutine runtimes (per round) for different datasets. }
\end{table}


\subsection{Regret Minimization}
For our regret minimization experiments, we compare CUCB, $\epsilon$-greedy, initial exploration, pure exploitation and random seed selection. for $\epsilon$-greedy,  we set the parameter $\omega = 5$ and for initial exploration we set $\zeta = 0.2$. For CUCB, if the update results in any $\mu_{i}$ exceeding 1, we reset it back to 1. All the probabilities are initialized to $0$. We show results on the NetHept and Epinions datasets for $k = 50$ for both the node level and edge level feedback mechanism. Results for other $k$ and the Flickr dataset are similar. 

Figure~\ref{fig:nethept-50-regret} shows the decrease in average regret as the number of rounds increase. We see that convergence for the CUCB algorithm is slow. This is because a UCB based algorithm is biased towards exploring edges which have not been triggered enough number of times(or even once). Since typical networks 	consist of a large number of edges, the rate of decrease in regret for the CUCB algorithm is slow. This behaviour is observed for other datasets as well. Hence we do not show results for the CUCB algorithm in subsequent plots. 


For all datasets, for other algorithms such as $\epsilon$-greedy and initial exploration, we can control the amount of exploration by the parameters $\omega$ and $\zeta$. For these algorithms, 
it can be seen from figures~\ref{flickr-50-regret,epinions-50-regret}, we see that the regret decreases at a much faster rate almost tending to zero in $1000$ rounds. This implies that at the end of $1000$ rounds, the learnt probabilities have been estimated well enough to lead to a comparable influence as against the known probabilities. For initial exploration, we see that the regret remains almost the same during the exploration phase in the first $200$ rounds of the algorithm. Average regret at the end of $1000$ rounds is minimum for pure exploitation. This is not uncommon and for cases such as our where the rewards are noisy such as ours, exploiting and choosing the best superarm greedily often leads to best results.  We also observe that the edge level and node level feedback mechanisms achieve almost the same regret in all cases and hence this leads to infer that the failure probability is indeed low for typical social networks. In fact, we can use equation~\ref{eq:failure-probability} to find the failure probability. For the NetHept dataset, the average number of active parents$K$ for a node is $1.175$. Hence credit distribution is not a big issue. If $p_{min} = 0$ and $p_{max}$ varies from $0.01$ to $0.2$, the failure probability $\rho$ varies from $0.0115$ to $0.2261$. Previous literature has shown that the probabilities learnt from diffusion traces are generally small. Hence the failure probability of the proposed node level feedback mechanism is small. We obtain similar results on the Epinions and Flickr datasets as well. 

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{./figs/Nethept/50-L2-Error.png}
\caption{NetHept, $k$ = 50: L2 error vs Number of Rounds for different algorithms}
\label{fig:nethept-50-L2-error}
\end{figure}

For NetHept, we plot the relative L2 error for the influence probabilities in Figure ~\ref{fig:nethept-50-L2-error}. As the rounds progress, the mean estimates improve and the relative L2 error goes down. This leads to better estimates of expected spread, the quality of the chosen seeds improves, the true spread increases and hence the average regret goes down. We can see that although pure exploitation led to the best regret, it narrowed down on the seed set to be chosen quickly and did not learn about the other edges in the network. $\epsilon$-greedy and initial exploration however did a fair bit of exploration and hence have a lower L2 error. However, for the larger datasets pure exploitation explores the network more before settling on a seed set. Hence, the L2 error is as small as the other algorithms. 

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{./figs/Epinions/k-effect.png}
\caption{Epinions, Average spread vs $k$}
\label{fig:epinions-k-effect}
\end{figure}
We observe the effect of changing $k$ in Figure~\ref{fig:epinions-k-effect}. We plot the average spread obtained using the learnt probabilities in across the rounds. We observe that the failure probability is small irrespective of the seed budget and the spread obtained using node level feedback is always close to that using edge level feedback. We can also observe the effect of submodularity i.e. the slope of the graph decreases as $k$ increases. 

%For our final experiment, we observe the effect of adding a prior. In particular, we compare the regret obtained by using a beta prior characterized by parameters $(1,9)$ to the regret obtained without prior for NetHept, $k = 50$ and the $\epsilon$-greedy strategy under both feedback mechanisms. 
%
%\begin{figure}
%\centering
%%\includegraphics[scale=0.3]{./figs/Nethept/prior-effect.png}
%\label{fig:nethept-prior-effect}
%\end{figure}


\subsection{Network Exploration}
We show results for the Nethept dataset, with $k = 50$ and a beta prior of $(1,9)$. Since we want to learn the probabilities as quickly as possible, we warm start the learning by using domain specific knowledge.

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{./figs/Nethept/50-L2-Error-exp.png}
\caption{ NetHept, $k$ = 50, L2 Error vs Number of rounds }
\label{fig:nethept-50-L2-Error-exp}
\end{figure}

In figure~\ref{nethept-50-L2-Error-exp}, we compare the L2 error obtained by using random exploration and strategic exploration strategies coupled with Edge level feedback and both the frequentist and maximum likelihood based node level feedback mechanisms. First, we can see that using a strategic exploration strategy is better than just choosing nodes at random because it incorporates feedback from what happened in the previous rounds and explicitly tries to avoid those edges which have been sampled. We observe that the decrease in error for frequentist approaches is much quicker as compared to the maximum likelihood approach. It is expected that edge level feedback shows the fastest decrease in error. The frequentist node level feedback takes more aggressive steps as compared to the maximum likelihood approach which is a more principled and moderate approach towards distributing credit. However since the failure probability is low in typical networks, the aggressiveness for the frequentist approach pays off leading to a very quick decrease in error. 

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{./figs/Nethept/50-Fraction-exp.png}
\caption{NetHept, $k$ = 50, Fraction of edges within relative error of $10\%$ vs Number of rounds}
\label{fig:nethept-50-Fraction-exp}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{./figs/Nethept/50-Fraction-Thresholds-exp.png}
\caption{ NetHept, $k$ = 50, Fraction of edges within relative error of $p$ vs $p$ }
\label{fig:nethept-50-Fraction-Thresholds-exp}
\end{figure}

We also show the plot~\ref{fig:nethept-50-Fraction-exp} for fraction of edges which are within a relative error of $10\%$ of their true probabilities. In figure~\ref{fig:nethept-50-Fraction-Thresholds-exp}, we also plot a ROC-type curve which varies the amount of relative error that can be tolerated on the X axis and the fraction of edges within this precision. As expected, the fraction increases as the allowable error is increased. We see that a large percentage of edges lie within $20$ error thus verifying the effectiveness of our network exploration algorithms.
